Overcoming Reward Overoptimization via Adversarial Policy Optimization with Lightweight Uncertainty Estimation

We introduce Adversarial Policy Optimization (AdvPO), a novel solution to the pervasive issue of reward over-optimization in Reinforcement Learning from Human Feedback (RLHF) for Large Language Models (LLMs). Over-optimization occurs when a reward model serves as an imperfect proxy for human preference, and RL-driven policy optimization erroneously exploits reward inaccuracies. In this paper, we begin by introducing a lightweight way to quantify uncertainties in rewards, relying solely on the last layer embeddings of the reward model, without the need for computationally expensive reward ensembles. AdvPO then addresses a distributionally robust optimization problem centred around the confidence interval of the reward model's predictions for policy improvement. Through comprehensive experiments on the Anthropic HH and TL;DR summarization datasets, we illustrate the efficacy of AdvPO in mitigating the overoptimization issue, consequently resulting in enhanced performance as evaluated through human-assisted evaluation.

==> framework.tex <==
\section{Utilizing Uncertainty to Mitigate Reward OverOptimization}
\label{sec:advpo}

The lightweight uncertainty estimation also inspires a novel framework, \model{}, to address the issue of overoptimization during policy optimization. Instead of optimizing towards the potentially incorrect point estimate $r_{\varphi}(x,y)$, which may lead to overoptimization, \model{} optimizes the LLM policy towards the reward model's prediction confidence interval constructed in Eq.(\ref{inequ:bandit-un-new}), considering that the true reward could assume any value within the interval with equal probability.

\textbf{Connection between rewards and projection weights}: An important corollary to Theorem \ref{thm:ineq}, which will play a major part in the next section, is that the difference in rewards can in fact be upper bounded by the difference in projection weights. In other words, if the difference in the projection weights are bounded so is the difference in the rewards. Due to space constraints, the detailed derivation is provided in Appendix \ref{appendix-secthe}. At a high level, under the neural tangent kernel assumption and considering the linearity of rewards with respect to fixed embeddings \(r(x, y) = \phi^T e(x, y)\), we demonstrate that:
\begin{equation}
|r^*(x,y) - r_{\varphi}(x,y)| \leq U_{x,y}^{CI}\|\phi^* - \hat{\phi}\|_{M_D} \leq U_{x,y}^{CI} b_{D, \delta} 
\end{equation}
Here, \(\phi^*\) and \(\hat{\phi}\) represent the optimal and estimated projection weights for reward prediction, respectively.



% Given that the lightweight uncertainty estimation method in Section 3 capture the reliability of estimated rewards and demonstrate potential in mitigating the overoptimization issue, this section devises an effective way to leverage them in policy 
% optimization.


% The reward uncertainties enable the construction of a confidence interval containing the golden reward with high probability, as defined in Eq.(\ref{inequ:bandit-un-new}). 
% Consequently, to mitigate the risk of overoptimization caused by high rewards with high uncertainty, we should not solely optimize towards the potentially incorrect point estimate $r_{\varphi}(x,y)$.
%  Instead, it is imperative to optimize the policy towards the reward model's prediction confidence interval, considering that the gold reward could assume any value within the interval with equal probability.





Here, with a bit of abuse of notation, we use $r_{\phi}(\cdot)$ to denote the reward obtained when using the projection weight $\phi$, while keeping the representation encoder unchanged.

\begin{align}
 \textbf{(AdvPO)} ~~~~  \max_{\pi_{\theta}} & \min_{\small \|\phi - \hat{\phi}\|^2_{M_D} \leq B}  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\phi}(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ r_{\phi}(x,y_{\rm ref})\right] \nonumber \\
    & \quad - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
    \label{equ:opt-1}
\end{align}
\jef{maybe we can be more explicit here. I think this is the crux of the method and we should try to make this as easy to understand for the reader as possible. Maybe we can discuss this tmr as well.}


\textbf{Maxmin formulation using confidence interval} As discussed in Section \ref{subsec:un-cal}, once the confidence region of the projection weight $\hat{\phi}$ is established, sample-wise reward uncertainty or confidence interval is derived through additional relaxation using standard inequalities such as the Cauchy-Schwarz inequality.
For ease of illustration, we denote the confidence region of the projection weight $\hat{\phi}$ as: $\|\phi^* - \hat{\phi}\|_{M_D}^2 \leq B$ with $B= b_{D,\delta}^2$ in the subsequent discussion.
Thus, instead of optimizing toward the reward confidence interval for each sample individually,  \model{}  tackles the following distributionally robust optimization for policy improvement,  where the inner optimization directly seeks a pessimistic projection weight $\phi$ within the confidence ball for reward calculation:


\textbf{Reference baseline responses} To prevent \model{} from becoming overly pessimistic or optimizing incorrectly, we further integrate reference responses $\{y_{\rm ref}\}$ into the objective function.
As illustrated in Lemma \ref{lem:ref-effect}, incorporating reference responses encourages the policy to move towards the average embedding of these references, i.e., $ \mathbb{E}_{x, y_{\rm ref}}[ e(x,y_{\rm ref}) ]$.
By utilizing any acceptable reference responses, such as annotated good responses from users or outputs generated by the SFT model, the policy optimization is guided more accurately, preventing \model{} from being overly pessimistic or incorrect.

 \yl{state the theorem here}
Theorem \ref{thm:inner-min} in Appendix \ref{appendix-secthe}  demonstrates the inner minimization of Eq.(\ref{equ:opt-1}) has a closed-form solution, and thus the optimization problem in Eq.(\ref{equ:opt-1}) has an equivalent but easier to operate form:
 \begin{align}
    \max_{\pi_{\theta}} \quad &  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} [r_{\hat{\phi}}(x,y) - \frac{1}{\lambda^*} e(x,y)^\top M_D^{-1} g ]    - \mathbb{E}_{x, y_{\rm ref}} [r_{\hat{\phi}}(x,y_{\rm ref}) - \frac{1}{\lambda^*} e(x,y_{\rm ref})^\top M_D^{-1} g ] \nonumber \\
    & - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right], \label{equ:final-obj}
    \end{align}
where %$e(x,y)$ denotes the last layer embedding of the prompt-response pair $(x,y)$, and 
$g=\mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[e(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ e(x,y_{\rm ref}) \right]$ and $\lambda^* = \sqrt{\frac{g^\top M^{-1}g}{B}}$.

\jef{Lets discuss this part tmr. I think we should have an intuition paragraph here, where even when readers dont understand math should understand the main message/}

\noindent
\textbf{Comparison to previous approaches in utilizing uncertainty against overoptimization.}
Previous work \cite{coste2023reward, eisenstein2023helping,zhai2023uncertainty} utilizes reward uncertainty on a per-sample basis, i.e., penalizing each sample's reward based on its individual uncertainty, as illustrated in Eq.(\ref{equ:sw-un}).
While both per-sample uncertainty penalization and \model{} adopt a pessimistic approach to leveraging reward uncertainty, the degree of pessimism is crucial \cite{jin2021pessimism,rashidinejad2021bridging,zhai2023uncertainty}.   Excessive pessimism, i.e., penalizing rewards too heavily based on uncertainties, is known to impede the discovery of the correct direction for optimization, thus failing to find a good policy.

However, as discussed in Section \ref{subsec:un-cal}, the sample-wise uncertainty in Eq.(\ref{inequ:bandit-un-new}) is derived from the confidence region of the learned projection weight $\hat{\phi}$ through additional relaxations. \yl{state the theorem} Lemma \ref{lemma:conservative} in Appendix \ref{appendix-secthe}  shows that penalizing uncertainty on a sample-wise basis, as done in previous work \cite{coste2023reward, eisenstein2023helping,zhai2023uncertainty}, leads to a more pessimistic objective than the max-min objective in Eq.(\ref{equ:final-obj}) of \model{}. This indicates that \model{} is more effective in enhancing policy performance and reducing overoptimization.

% \model{} leverages uncertainty less pessimisticly, 





==> framework_jef.tex <==

\section{Utilizing Uncertainty to Mitigate Reward Overoptimization }
\label{sec:advpo}
This section introduces our framework, \model{}, to address the issue of overoptimization during policy optimization by leveraging the aforementioned lightweight uncertainty estimation.

Instead of optimizing towards a potentially incorrect point estimate \(r_{\hat{\varphi}}\), which causes overoptimization, \model{} aim to optimize the following \texttt{MaxMin} objective which takes into account the confidence region around the imperfect reward model $r_{\hat{\varphi}}$ that contains the ground-truth reward $r^*$:
\begin{align*}
\max_{\pi_{\theta}} & \min_{{\varphi \in C_{\delta}^r(\hat{\varphi})} } \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\varphi}(x, y) \right] - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}} \left[ \pi_{\theta}(y | x) \middle\| \pi_{\rm \small SFT}(y | x) \right] \right],
\end{align*}
Here, $C_{\delta}^r(\hat{\varphi})$ contains all possible $\varphi$ values centered around the current estimate $\hat{\varphi}$, but also includes the optimal $\varphi^*$ that yields the ground truth reward, with a probability of $1-\delta$.
% that yields the reward $r_{\varphi}(x,y)$  centerering around \(r_{\hat{\varphi}}\) but contains the groundtruth reward $r^*(x,y)$ with probaility $1-\delta$.
% such that $|r_{\varphi}(x,y) - r_{\hat{\varphi}}(x,y)|$ meets the upper bound in Eq. (\ref{inequ:bandit-un-new}).
% of the reward $r_{\varphi}$ derived through lightweight uncertainties. Concretely, we have the point-wise region defined as $C_b^{r_{\varphi}}(x,y) := [r_{\varphi}(x,y) - U_{x,y}^{CI}, r_{\varphi}(x,y) + U_{x,y}^{CI}]$ according to Eq. (\ref{inequ:bandit-un-new}).
Intuitively, \model{} aims to maximize the same objective as in standard PPO (Eq. \ref{eq:PPO}), while also adversarially searching for the pessimistic reward function within the predicted reward $r_{\hat{\varphi}}$'s confidence ball 
% while adversarially searching for the pessimistic reward within the ball around the predicted reward 
containing the ground-truth reward $r^*$.
However, this \texttt{MaxMin} objective poses some practical issues, 
%given that exhausting the whole parameter space to search for the reward model $r_{\varphi}(x,y)$
given the inner minimization over $C_{\delta}^r(\hat{\varphi})$
%minimization over all possible rewards $r$
is intractable. Hence \model{} makes the following observation.

\textbf{Connection between Rewards and Projection Weights:} 
An important corollary to Theorem \ref{thm:ineq}, crucial to \model{}, is that $U_{x,y}^{CI}$, the first term of the upper bound of the reward difference $|r^*(x,y) - r_{\varphi}(x,y)|$ in Eq.(\ref{inequ:bandit-un-new}), actually 
represents the uncertainty stemming from the inaccuracy in the estimated projection weight $\hat{\phi}$.

Recall that $e(x,y)$ denotes the last layer embedding of the prompt and response pair $(x,y)$.
Let \(\phi^*\) and \(\hat{\phi}\) be the optimal and estimated projection weights for reward prediction respectively.
Under the assumption mentioned in Section \ref{subsec:un-cal}, the ground-truth reward can be approximated by a linear function of optimal projection weight $\phi^*$ and  $e(x,y)$, plus a term that can be bounded, i.e., $r^*(x, y) = e(x, y)^\top\phi^*  + \text {bounded term}$.
Considering the linearity of rewards with respect to the last layer embeddings \(r_{\hat{\varphi}}(x, y) = \hat{\phi}^\top e(x, y)\), and denoting the established confidence region of the projection weight as  $\| \hat{\phi}-\phi^*\|_{M_D} \leq b$, we show that:
\begin{equation}
|r^*(x, y) - r_{\hat{\varphi}}(x, y)| 
\leq \underbrace{|e(x, y)^\top\phi^* - e(x, y)^\top\hat{\phi}| + \text{const} }_{A_1}
\leq \underbrace{\|\phi^* - \hat{\phi}\|_{M_D}  \sqrt{e(x,y)^\top M_D^{-1} e(x,y)}}_{ \leq U_{x,y}^{CI}} + \text{const} 
% \leq U_{x,y}^{CI}  + \text{const},
\label{eq:trans}
\nonumber
\end{equation}
% \textbf{Connection between Rewards and Projection Weights:} An important corollary to Theorem \ref{thm:ineq}, which is crucial to \model{}, is that the difference in rewards, i.e., $|r^* - r_{\varphi}|$, which determines the confidence interval of rewards $C^r_b(\cdot, \cdot)$, can be upper-bounded through relaxations based on the confidence region of projection weights.
% Specifically, once the confidence region of projection weights is established, the difference in rewards can also be bounded,  the detailed derivation is provided in Appendix \ref{appendix-secthe}.
% Recall that $e(x,y)$ denotes the last layer embedding of prompt and response pair $(x,y)$.
% At a high level, let \(\phi^*\) and \(\hat{\phi}\) be the optimal and estimated projection weights for reward prediction, respectively.
% Given the confidence region  $\| \hat{\phi}-\phi^*\|_{M_D} \leq b$, under the assumption mentioned in Section \ref{subsec:un-cal}, the ground-truth reward can be approximated by a linear function of optimal projection weight $\phi^*$ and  $e(x,y)$, plus a term that can be bounded, i.e., $r^*(x, y) = e(x, y)^T\phi^*  + \text {bounded term}$.
% Considering the linearity of rewards w.r.t  last layer embeddings  \(r_{\varphi}(x, y) = \hat{\phi}^T e(x, y)\), we show that:
% \begin{equation}
% |r^*(x, y) - r_{\varphi}(x, y)| 
% \leq |e(x, y)^T\phi^* - e(x, y)^T\hat{\phi}| + \text{const} 
% \leq \|\phi^* - \hat{\phi}\|_{M_D} \cdot \sqrt{e(x,y)^\top M_D^{-1} e(x,y)}
% %+ \text{const}\leq U_{x,y}^{CI}  + \text{const},
% \nonumber
% \end{equation}
Therefore, the objective of the inner optimization problem in \model{} can be relaxed to optimize an upper bound, i.e., $A_1$ in Eq. (\ref{eq:trans}), where the minimization is now taken over the projection weights instead of the reward functions.
\begin{align}
 \max_{\pi_{\theta}} & \min_{{\small \|\phi - \hat{\phi}\|_{M_D} \leq b}}  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\phi}(x, y) \right] - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}} \left[ \pi_{\theta}(y | x) \middle\| \pi_{\rm \small SFT}(y | x) \right] \right],
    \label{equ:opt-1}
\end{align}
Here, with a bit of abuse of notations, we use $r_{\phi}(\cdot)$ to denote the reward obtained when using the projection weight $\phi$, while keeping the representation encoder unchanged.

It is important to note that this approach diverges significantly from conventional reward penalization methods \cite{coste2023reward, eisenstein2023helping, zhai2023uncertainty}. Rather than focusing on the worst-case scenario for each sample, our objective function adopts a more holistic perspective by minimizing across the reward functions themselves. Further details on the differences will be elaborated later in this section (Lemma \ref{lemma42}).

\textbf{Incorporating Reference Responses.} To prevent \model{} from becoming overly pessimistic, we introduce reference responses $\{y_{\rm ref}\}$ into the objective, resulting in the final objective of \model{}:
\begin{align}
 \textbf{(AdvPO)} ~~~~  \max_{\pi_{\theta}} & \min_{\small \|\phi - \hat{\phi}\|_{M_D} \leq b}  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\phi}(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ r_{\phi}(x,y_{\rm ref})\right] \nonumber \\
    & \quad - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
    \label{equ:opt-1}
\end{align}

As illustrated in Lemma \ref{lem:ref-effect}, incorporating reference responses enforces policy optimization towards the direction of the reference responses, i.e., $ \mathbb{E}_{x, y_{\rm ref}}[ e(x,y_{\rm ref}) ]$,  while optimizing against pessimistic rewards.
Thus as long as the set of reference responses is reasonably good and achieves a positive ground-truth reward on average, i.e, $ (\mathbb{E}_{x, y_{\rm ref}}[ e(x,y_{\rm ref}) ])^\top \phi^* >0$, the policy is guided to outperform the reference, preventing \model{} from being overly pessimistic.
In practice, the reference responses can be any acceptable answers, such as annotated good responses from users or responses generated by the SFT policy.
% By utilizing any acceptable reference responses, such as annotated good responses from users, the policy optimization is guided more accurately, preventing \model{} from being overly pessimistic or incorrect.




Next, we show in Theorem \ref{thm:inner-min} that the inner minimization of Eq.(\ref{equ:opt-1}) has a closed-form solution and hence Eq.(\ref{equ:opt-1}) reduces to an objective function that can be optimized using standard gradient ascent. 


% \begin{theorem}
%     The optimization problem in Eq.(\ref{equ:opt-1}) is is equivalent to the following objective:
%     \begin{align*}
%         \max_{\pi_{\theta}} \quad  &  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} [r_{\phi}(x,y) - \frac{1}{\lambda^*} e(x,y)^T M_D^{-1} g ] - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
%     \end{align*}
%     where  $e(x,y)$ denotes the last layer embedding of the prompt-response pair $x$ and $y$, and $g=\mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[e(x,y)\right]$, and $\lambda^* = \sqrt{\frac{g^TM^{-1}g}{B}}$.
%     \label{thm:inner-min1}
% \end{theorem}

% Theorem \ref{thm:inner-min} in Appendix \ref{appendix-secthe}
\begin{theorem}
    The optimization problem in Eq.(\ref{equ:opt-1}) is equivalent to the following objective:
 \begin{align}
    \max_{\pi_{\theta}} \quad &  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} [r_{\hat{\phi}}(x,y) - \frac{1}{\lambda^*} e(x,y)^\top M_D^{-1} g ]    - \mathbb{E}_{x, y_{\rm ref}} [r_{\hat{\phi}}(x,y_{\rm ref}) - \frac{1}{\lambda^*} e(x,y_{\rm ref})^\top M_D^{-1} g ] \nonumber \\
    & - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right], \label{equ:final-obj}
    \end{align}
where $e(x,y)$ denotes the last layer embedding of the prompt-response pair $(x,y)$, and 
$g=\mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[e(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ e(x,y_{\rm ref}) \right]$ and $\lambda^* = \sqrt{\frac{g^\top M^{-1}g}{b^2}}$.
 \label{thm:inner-min}
\end{theorem}

Theorem \ref{thm:inner-min} shows that the initial \texttt{MaxMin} objective can be loosened and rewritten into a standard \texttt{Max} objective for which we can use standard gradient ascent. %Note that $M^{-1}_D \in \mathbb{R}^d \times \mathbb{R}^d$, where $d$ is the representation dimension and can be precomputed, thus not posing a computational bottleneck.


% \yl{this paragraph below now reads redundant}
% \textbf{Maxmin formulation using confidence interval} As discussed in Section \ref{subsec:un-cal}, once the confidence region of the projection weight $\hat{\phi}$ is established, sample-wise reward uncertainty or confidence interval is derived through additional relaxation using standard inequalities such as the Cauchy-Schwarz inequality.
% For ease of illustration, we denote the confidence region of the projection weight $\hat{\phi}$ as: $\|\phi^* - \hat{\phi}\|_{M_D}^2 \leq B$ with $B= b_{D,\delta}^2$ in the subsequent discussion.
% Thus, instead of optimizing toward the reward confidence interval for each sample individually,  \model{}  tackles a distributionally robust optimization for policy improvement,  where the inner optimization directly seeks a pessimistic projection weight $\phi$ within the confidence ball for reward calculation.




%  \yl{state the theorem here}
% Theorem \ref{thm:inner-min} in Appendix \ref{appendix-secthe}  demonstrates the inner minimization of Eq.(\ref{equ:opt-1}) has a closed-form solution, and thus the optimization problem in Eq.(\ref{equ:opt-1}) has an equivalent but easier to operate form:
% Thus the final objective can be written as follows, for all the details and derivations we refer the reader to Appendix \ref{appendix-secthe}:
%  \begin{align}
%     \textbf{(AdvPO)} ~~~~~ &\max_{\pi_{\theta}} ~  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} [r_{\hat{\phi}}(x,y) - \frac{1}{\lambda^*} e(x,y)^\top M_D^{-1} g ]   \\& - \mathbb{E}_{x, y_{\rm ref}} [r_{\hat{\phi}}(x,y_{\rm ref}) - \frac{1}{\lambda^*} e(x,y_{\rm ref})^\top M_D^{-1} g ] \nonumber \\
%     & - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
%     \end{align}
% where %$e(x,y)$ denotes the last layer embedding of the prompt-response pair $(x,y)$, and 
% $g=\mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[e(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ e(x,y_{\rm ref}) \right]$ and $\lambda^* = \sqrt{\frac{g^\top M^{-1}g}{B}}$.

% \jef{Lets discuss this part tmr. I think we should have an intuition paragraph here, where even when readers dont understand math should understand the main message/}

\noindent
\textbf{Comparison to previous approaches in utilizing uncertainty against overoptimization.}
As mentioned above, recent works \cite{coste2023reward, eisenstein2023helping,zhai2023uncertainty} utilize reward uncertainty on a per-sample basis, i.e., penalizing each sample's reward based on its individual uncertainty, as illustrated in Eq.(\ref{equ:sw-un}).
While both per-sample uncertainty penalization and \model{} adopt a pessimistic approach to leverage reward uncertainty, the degree of pessimism is crucial \cite{jin2021pessimism,rashidinejad2021bridging,zhai2023uncertainty}. Excessive pessimism, i.e., penalizing rewards too heavily based on uncertainties, is known to impede the discovery of the correct direction for optimization, thus failing to find a good policy. To demonstrate this, we prove the following:
\begin{lemma} \label{lemma42}
Compared with the sample-wise uncertainty penalization used in \cite{coste2023reward, eisenstein2023helping}, the distributionally robust
optimization objective of \model{} in Eq. (\ref{equ:opt-1}) utilizes uncertainty less conservatively.
\label{lemma:conservative}
\vspace{-6mm}
\end{lemma}
This demonstrates that \model{} is more effective in enhancing policy performance while reducing over-optimization, which we will back up with extensive large-scale experiments in the next section.
% However, as discussed in Section \ref{subsec:un-cal}, the sample-wise uncertainty in Eq.(\ref{inequ:bandit-un-new}) is derived from the confidence region of the learned projection weight $\hat{\phi}$ through additional relaxations. \yl{state the theorem} Lemma \ref{lemma:conservative} in Appendix \ref{appendix-secthe}  shows that penalizing uncertainty on a sample-wise basis, as done in previous work \cite{coste2023reward, eisenstein2023helping,zhai2023uncertainty}, leads to a more pessimistic objective than the max-min objective in Eq.(\ref{equ:final-obj}) of \model{}. This indicates that \model{} is more effective in enhancing policy performance and reducing overoptimization.

==> framework_revised.tex <==
\section{Revised Part of Section 3}
\paragraph{Uncertainty Quantification in Neural Bandits.}


Following previous work \cite{xu2020neural, riquelme2018deep},{\color{blue} we demonstrate in Theorem \ref{appendix:un-derive} } that 
with probability $1-\delta$, the following inequality concerning the uncertainty, or the width of the confidence interval of the estimated reward, holds:
\begin{align}
    |r^*(x,y) - r_{\varphi}(x,y)| \leq b \sqrt{e(x,y)^\top M_D^{-1} e(x,y)},
    \label{inequ:bandit-un}
\end{align}
where $b$ is a function of $\delta$ (typically the smaller $\delta$ is, the larger $b$ is). 
And $M_D$ summarizes all last layer embeddings observed in the training data for the reward model, i.e.,{\color{blue} $M_D =  \lambda I + \sum_{i=1}^N \sum_{y \in \{y_c^i, y_r^i\}} e(x_i,y) e(x_i,y)^\top $. }For ease of illustration, we then denote $U_{x,y}^{CI}=\sqrt{e(x,y)^\top M_D^{-1} e_(x,y)}$.
Intuitively, if the new prompt-response pair $(x, y)$ is similar to samples in the training data, applying the inverse of $M_D$ would result in a small uncertainty $U_{x,y}^{CI}$; otherwise, the uncertainty will be high.


\section{Revised Version of Section 4}
Given that the lightweight uncertainty estimation methods in Section 3 capture the reliability of estimated rewards and demonstrate potential in mitigating the overoptimization issue, this section devises an effective way to leverage them to improve policy optimization. For subsequent sections, we primarily adopt CI in Eq.(\ref{inequ:bandit-un}) to quantify uncertainties in reward modelling, as it demonstrates strong effectiveness, as shown in Figure 1.


The reward uncertainties enable the construction of a confidence interval containing the golden reward with high probability, as defined in Eq.(\ref{inequ:bandit-un}). 
{\color{blue}
Consequently, to mitigate the risk of overoptimization caused by high rewards with high uncertainty, we should not solely optimize towards the potentially incorrect point estimate $r_{\varphi}(x,y)$.
 Instead, it is imperative to optimize the policy towards the reward model's prediction confidence interval, considering that the gold reward could assume any value within the interval with equal probability.


As derived in Theorem \ref{appendix:un-derive}, the reward confidence interval indeed arises from the confidence region of the projection weight $\hat{\phi}$, expressed as $\|\phi^* - \hat{\phi}\|_{M_D}^2 \leq B$, where $\phi^* \in \mathbb{R}^d$ and $\hat{\phi} \in \mathbb{R}^d$ denote the optimal and estimated projection weights for the last layer to predict rewards, respectively.

Thus, instead of optimizing toward the reward confidence interval for each sample individually, \model{} employs distributionally robust optimization, where the inner optimization directly seeks a pessimistic projection weight $\phi$ within the confidence ball for reward calculation,
}
\begin{align}
    \max_{\pi_{\theta}} & \min_{\small \|\phi - \hat{\phi}\|^2_{M_D} \leq B}  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\phi}(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ r_{\phi}(x,y_{\rm ref})\right] \nonumber \\
    & \quad - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
    \label{equ:opt-1}
\end{align}
Here, with a bit of abuse of notation, we use $r_{\phi}(\cdot)$ to denote the reward obtained when using the projection weight $\phi$, while keeping the representation encoder unchanged.


% As the lightweight uncertainty estimation focuses solely on the last layer embeddings, the reward uncertainty implies uncertainty in the learnt projection weight in the reward model. Specifically, let $\phi^* \in \mathbb{R}^d$ and $\hat{\phi} \in \mathbb{R}^d$ denote the optimal and estimated projection weights for the last layer to predict rewards, respectively. We have that: $\exists B \in \mathbb{R}_+, \|\phi^* - \hat{\phi}\|_{M_D}^2 \leq B$ (Lemma C.4 \cite{xu2020neural}). Recall that $M_D$ summarizes all last layer embeddings observed during the training of the reward model and can thus be precomputed.


% Within the confidence interval of learnt projection weight, \model{} searches for reward predictions that are most pessimistic about the current policy and then improve the policy against such rewards. Since the gold reward is guaranteed to be covered by the confidence interval with high probability, using the most pessimistic reward (i.e., the lowest possible reward) naturally avoids over-optimization. Formally, this formulates a distributionally robust optimization problem, 
% \begin{align}
%     \max_{\pi_{\theta}} & \min_{\small \|\phi - \hat{\phi}\|^2_{M_D} \leq B}  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ r_{\phi}(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ r_{\phi}(x,y_{\rm ref})\right] \nonumber \\
%     & \quad - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right],
%     \label{equ:opt-1}
% \end{align}
% Here, with a bit of abuse of notation, we use $r_{\phi}(\cdot)$ to denote the reward obtained when using the projection weight $\phi$, while keeping the representation encoder unchanged.
%The hyperparameter $\beta$ still controls the extent of KL divergence regularization.


Furthermore, to better align our adversarial search with how the reward model is obtained in Eq. (1), we also incorporate a reference response through pairwise preference comparison in our objective function. 
The reference response can be any acceptable answer, such as an annotated good response from users or a response generated by the SFT model. 
{\color{blue}
As demonstrated in Lemma \ref{lem:ref-effect}, the inclusion of reference responses prevents AdvPO from becoming overly pessimistic or optimizing incorrectly. This is achieved by directing policy optimization toward the reference responses while also optimizing against pessimistic rewards.
}

Theorem D.1 in Appendix D demonstrates the inner minimization of Eq.(\ref{equ:opt-1}) has a closed-form solution, and thus the optimization problem in Eq.(\ref{equ:opt-1}) has an equivalent but easier to operate form:
 \begin{align}
    \max_{\pi_{\theta}} \quad &  \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} [r_{\hat{\phi}}(x,y) - \frac{1}{\lambda^*} e(x,y)^\top M_D^{-1} g ]   \label{equ:final-obj} \\
    & - \mathbb{E}_{x, y_{\rm ref}} [r_{\hat{\phi}}(x,y_{\rm ref}) - \frac{1}{\lambda^*} e(x,y_{\rm ref})^\top M_D^{-1} g ], \nonumber \\
    & - \beta \mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[ \mathbb{D}_{\text{KL}}\left[\pi_{\theta}(y|x) \middle\| \pi_{\rm \small SFT}(y|x)\right] \right], \nonumber
    \end{align}
where %$e(x,y)$ denotes the last layer embedding of the prompt-response pair $(x,y)$, and 
$g=\mathbb{E}_{x, y \sim \pi_{\theta}(\cdot | x)} \left[e(x,y)\right] - \mathbb{E}_{x, y_{\rm ref}}\left[ e(x,y_{\rm ref}) \right]$ and $\lambda^* = \sqrt{\frac{g^\top M^{-1}g}{B}}$.


\noindent
\textbf{Comparison to previous approaches in utilizing uncertainty against overoptimization.}
Previous work \cite{coste2023reward, eisenstein2023helping} utilizes reward uncertainty on a per-sample basis, i.e., penalizing each sample's reward based on its individual uncertainty, as illustrated in Eq. (3).
While both per-sample uncertainty penalization and \model{} adopt a pessimistic approach to leveraging reward uncertainty, the degree of pessimism is crucial \cite{jin2021pessimism,rashidinejad2021bridging}.   Excessive pessimism, i.e., penalizing rewards too heavily based on uncertainties, is known to impede the discovery of the correct direction for optimization, thus failing to find a good policy.

{\color{blue}
In Lemma D.2 of Appendix D, we theoretically demonstrate that directly penalizing uncertainty in a sample-wise manner, as in previous work \cite{coste2023reward, eisenstein2023helping}, results in a more pessimistic objective compared to the max-min objective in Eq.(\ref{equ:final-obj}) of \model{}. }
This suggests that \model{} is more likely to contribute to improving policy performance while mitigating overoptimization.

% \model{} leverages uncertainty less pessimisticly, 





















==> uncertainty_eval.tex <==
Since our objective is to harness uncertainty in reward modelling to mitigate the overoptimization issue in RLHF, we specifically examine whether the quantified uncertainties can identify discrepancies between estimated proxy rewards and gold rewards during the RL stage. 
We adopt a synthetic setup widely used in the literature \cite{gao2023scaling,coste2023reward, eisenstein2023helping}, where we train a significantly larger ``\textit{gold-standard}" reward model that simulates human preferences and provides labels for training a proxy reward model.


We run a standard RLHF pipeline on the Anthropic HH \cite{bai2022training} and TL;DR dataset\cite{stiennon2020learning}, with reward and policy models established from LLama-7B \cite{touvron2023llama}.
The preference dataset is labelled by the gold reward model. In particular, for the Anthropic HH dataset, the gold reward model is trained from Vicuna-13B \cite{platzer_et_al:LIPIcs.ECRTS.2021.1}, and for the TL;DR dataset, the gold reward model is trained from LLama-13B \cite{touvron2023llama}. Additional details, such as gold/proxy reward model training, PPO implementation, etc., can be found in Appendix \ref{appedix:exp-syn}.
% experimental procedurefor gold reward training 

% To simulate the fact that in a real setup, human preferences are too
% complex to be captured by a neural network with a finite
% capacity, we employ larger LLMs to get the gold reward models following previous work[ref]. 

During the PPO training stage, we log the generated samples every 10 steps. Subsequently, we compute their gold reward, proxy reward, as well as reward uncertainties associated with the proxy reward.
We compare the following uncertainty methods: 
\squishlist
 \item \textbf{CI}: 
 The proposed uncertainty quantification method in Eq.(\ref{inequ:bandit-un-new}); 
\item \textbf{ENS-7B}:  Ensemble of three LLama7B reward models; 
\item \textbf{ENS-3B}: Ensemble of three 3B reward models based on OpenLLaMA3B\_v2 \cite{openlm2023openllama}. Since there are no officially released 3B models for LLaMA, we adopt OpenLLaMA \cite{openlm2023openllama} which is an open-source smaller reproduction of Meta AI’s LLaMA, showcasing comparable performance.
\squishend

The results are presented in Figure \ref{fig:un}. In Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff}, we depict the correlation between derived uncertainty\footnote{Uncertainties calculated by different methods have different scales, so we normalized them to (0,1) for ease of comparison.} and the difference between gold reward and proxy reward (i.e., $|r^*(x,y) - r_{\varphi}(x,y)|$). Ideally, an effective uncertainty measure should increase as the difference between gold and proxy reward increases.
In Figure \ref{fig:hh-un-step} and Figure \ref{fig:tldr-un-step}, we illustrate the progression of proxy rewards (blue dashed line), gold rewards (blue solid line), and uncertainties calculated by two lightweight uncertainty estimation methods, along with ENS-3B, 
throughout the PPO optimization steps. The reward values are indexed on the left y-axis, while the uncertainty is indexed on the right y-axis. These figures provide insight into whether the calculated uncertainties can effectively recognize the over-optimization issue.

Our key insights are summarized as follows:

\begin{figure*}[t]
  \centering
  % \vspace{-5mm}
  \subfloat[Anthropic HH (Step)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/ANT_UN_step.png}
             \label{fig:hh-un-step}}
    \subfloat[Anthropic HH (Reward Diff)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/ANT_UN_reward_diff.png}
             \label{fig:hh-un-rewarddiff}}
   \subfloat[TL;DR (Step)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/TLDR_UN_step.png}
             \label{fig:tldr-un-step}}
  \subfloat[TL;DR (Reward Diff)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/TLDR_UN_reward_diff.png}
             \label{fig:tldr-un-rewarddiff}}
% \vspace{-1mm}
    \caption{Comparison among lightweight uncertainty estimations. In Figure \ref{fig:hh-un-step} and \ref{fig:tldr-un-step}, the blue lines with shaded areas depict the reward dynamics concerning optimization steps in PPO, where the solid and dashed lines represent gold and proxy rewards, respectively. The lines with dots denote the results from different uncertainty estimation methods. The reward values are indexed on the left y-axis, while the uncertainty is indexed on the right y-axis. In Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff}, we plot the correlation between uncertainty and the difference between gold reward and proxy reward.}
    \label{fig:un}
% \vspace{-4mm}
\end{figure*}


\noindent\textit{$\bullet$ The lightweight uncertainty estimation methods are effective in signalling over-optimizaton.} 
We observe from Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff} that, as the difference between gold reward and proxy reward increases, the uncertainty calculated by CI also rises. This demonstrates CI  indeed captures information on when the proxy reward is drifting away from the ground-truth reward. 
Furthermore, in Figure \ref{fig:hh-un-step} and \ref{fig:tldr-un-step}, it is evident that when there is a divergence between golden and proxy rewards, indicating over-optimization, the uncertainty calculated by CI  generally increases with the optimization steps. This suggests the potential to leverage them to address the over-optimization issue. 
% CI appears to outperform GP since it consistently increases with the divergence of gold and proxy rewards, while GP tends to stabilize after roughly $500$ steps, as shown in Figure \ref{fig:tldr-un-step}.



\noindent\textit{$\bullet$ The lightweight uncertainty estimation surpasses reward ensembles with comparable parameter sizes. }  Compared to CI,  ENS-3B appears to be less correlated with the divergence between gold and proxy rewards, particularly on the TL;DR dataset \cite{stiennon2020learning}. Unlike our methods,  the uncertainty calculated by ENS-3B does not exhibit a monotonically increasing trend with the reward difference between gold and proxy rewards. This is likely due to the fact the smaller reward models, in this case, 3B models, are not able to capture the preference well, thus leading to worse predictions.


In addition to CI, we empirically evaluate Bayesian uncertainty modeling on last layer embeddings to quantify reward uncertainty. Further implementation details and experimental results are provided in Appendix \ref{}
\xy{@Jef, can you help on organizing GP parts in appendix?}


==> uncertainty_old.tex <==
\section{Lightweight Uncertainty Estimation}
\label{sec:un}
In this section, we introduce the lightweight uncertainty estimation method, based solely on the final layer embeddings of a reward model. We start by offering a high-level intuition on why the last layer embedding captures essential information about uncertainties in the model's predictions. Following this, we present our lightweight uncertainty estimation method and evaluate its effectiveness.


\subsection{Connection between last layer embeddings and reward uncertainty}
% \jef{YANG COMMENT: TODO coverage on references}
% We start with a high-level intuition about why the last layer embeddings of a reward model are capable on deriving the model's output uncertainties.
We first explore a high-level intuition about how the final layer embeddings of a reward model can facilitate the estimation of uncertainties in the model's output.

As discussed in Section \ref{subsec:rlhf}, reward modelling can be decomposed into two parts: (1) learning a good representation $e(x, y)$ for the prompt and response pair through a pre-trained LLM; (2) projecting the learnt representation to yield a scalar reward using a mapping $\phi$.
For the first part, Very importantly, the training of LLMs on extensive text corpora, coupled with their vast number of parameters, enables these models to develop versatile representations that can even be used in zero/few-shot tasks \cite{min2023recent,wei2022emergent,brown2020language}, which demonstrate the adaptability of these representations.

However, the second part, which involves learning the projection weight $\phi$, is strictly tied to the preference data provided during the reward model training. 
Consequently, the reliability of rewards is closely linked to the accuracy and adaptability of the projection weight.
% Consequently, the generalizability of the evaluated rewards is closely linked to the accuracy and adaptability of the projection weight. 
% \jef{@XY can you please take a look at this sentence above. I am really not sure how to rewrite or whether this can be cut}

The above claim has been widely supported in previous work in deep neural networks \cite{chen2020simple, kirichenko2022last, riquelme2018deep, xu2020neural}.
For instance, \cite{kirichenko2022last, Labonte2023towards, lee2023surgical} demonstrate that by freezing the network up to its last layer and retraining only the projection head with a smaller data set,  where spurious correlation is absent, it can greatly improve robustness of the neural network model against these spurious correlations.
In the context of language models, recent experiments on weak-to-strong generalization \cite{burns2023weak} further reinforce this claim. 
Their findings reveal that, despite the fine-tuning of an LLM's last layer embedding with noisy labels from weak supervision, the model can still excel in later classification tasks if the projection weight is accurately derived from ground-truth labels. This highlights the adaptability and the rich information encapsulated in the last layer representation, accessible through simple projection weights.
% Building the understanding on generalized representation but restricted projection weights, we now turn to the role of a neural network model's last layer in uncertainty quantification. \jef{need to reword this sentence}

Building upon the notion of generalized representations with specialized projection weights, we now shift our focus to the last layer's ability for uncertainty estimation. The projection weight is strictly estimated based on the preference data encountered during reward model training.
Therefore, when evaluating the prompt and response pairs during the RL stage, the pairs might deviate from what was observed during reward training (suggesting it undergo distribution shift \cite{wang2024secrets}), hence rendering the predicted rewards unreliable as they might be outside the support of training set.
To this end, we show in the next section how the last layer embedding of a reward model, based on preference data, can act as a feature map for an underlying kernel.
This kernel then allows us to determine whether new prompt response pairs are similar to the ones seen during training.
If not, the corresponding uncertainty should be higher, and therefore penalized during policy optimization.

% . This similarity measure then allows us to assess how new prompt-response pairs compare to those encountered during training, i.e., less similar embeddings imply higher uncertainty, while highly similar embeddings suggests lower uncertainty. 



% the last layer embedding of a reward model (on preference data) defines a feature maps for given kernel (similarity measure). This kernel then allows us to determine whether new prompt response pairs are similar to the ones we have seen during training. If not the associated uncertainty should be higher, If yes then the uncertainty should be lower


% a kernel space measuring the support of the model's span \jef{we need to be more precise here. Do we mean that the embeddings defines a feature map which corresponds to a RKHS?} \xy{I think it's okay, no need to be pretty specific here just for high intuition.}.
% Then the distance between the embedding of newly inputted prompt and response pair to this space quantifies the uncertainty associated  with the predicted reward.


% The adoption of last layer embeddings in neural networks has gained significant traction, particularly due to their rich representational power, computational efficiency and ease of use \cite{chen2020simple, kirichenko2022last, riquelme2018deep, xu2020neural}. For instance, \cite{kirichenko2022last, Labonte2023towards, lee2023surgical} demonstrate that by freezing the network up to its last layer and retraining only this layer, it is possible to effectively address spurious correlations issues, i.e. one of the causes of overoptimization. 

% Furthermore, in the context of language models, \cite{burns2023weak} showed that retraining just the last layer on a weak language model (trained on noisy data), using high-quality labels from a more sophisticated model, significantly elevates its performance. These finding suggests that last layer embeddings are versatile representations of the underlying data distribution and contain easily extractable information through simple linear transformation.

\subsection{Uncertainty via Last Layer Embeddings}
\label{subsec:un-cal}

Many methods for quantifying uncertainty in a neural network's output, derived from the model's final layer embeddings, have demonstrated their effectiveness both in theory and in practice \cite{xu2020neural, riquelme2018deep}. 
In this work, we take a closer look at the following two methods due to their
computational efficiency and theoretical soundness. 
\paragraph{Uncertainty Quantification in Neural Bandits.}

Previous work \cite{xu2020neural, riquelme2018deep} demonstrated that 
%performing an upper confidence bound (UCB)-type exploration on the projection layer of the network can effectively addresses the exploration-exploitation dilemma. They show that 
with probability $1-\delta$, the following inequality concerning the uncertainty, or the width of the confidence interval of the estimated reward, holds:
\begin{align}
    |r^*(x,y) - r_{\varphi}(x,y)| \leq b \sqrt{e(x,y)^\top M_D^{-1} e(x,y)},
    \label{inequ:bandit-un}
\end{align}
where $b$ is a function of $\delta$ (typically the smaller $\delta$ is, the larger $b$ is). 
And $M_D$ summarizes all last layer embeddings observed in the training data for the reward model, i.e., $M_D = \sum_{i=1}^N \sum_{y \in \{y_c^i, y_r^i\}} e(x_i,y) e(x_i,y)^\top$. 
For ease of illustration, we then denote $U_{x,y}^{CI}=\sqrt{e(x,y)^\top M_D^{-1} e_(x,y)}$.
Intuitively, if the new prompt-response pair $(x, y)$ is similar to samples in the training data, applying the inverse of $M_D$ would result in a small uncertainty $U_{x,y}^{CI}$; otherwise, the uncertainty will be high.

 
% Building on this understanding of last layer embeddings, we now turn to their role in uncertainty quantification. Empirical studies \cite{riquelme2018deep, xu2020neural} indicate that separating representation learning from uncertainty estimation can improve overall model performance when it comes to calibrated uncertainty quantification. For instance, \cite{xu2020neural} drew on bandit literature to establish Upper Confidence Bound (UCB) using only the last layer embeddings in the setting of contextual bandits. From a Bayesian perspective, \cite{wilson2016deep} proposed employing a Gaussian Process (GP) with last layer features as inputs for regression and classification tasks. Similarly, \citep{riquelme2018deep} and \citep{xu2020neural} applied Bayesian linear regression in their prediction tasks using last layer embeddings to a variety of contextual bandit problems. In each of the above problem settings, the uncertainty derived from only the last layer was on par with state-of-the-art methods thus demonstrating its potential in the realm of LLMs. 

% Nevertheless, a reasonable question to ask is: Why the last layer and not any other layer? To answer this, \cite{lee2023surgical} showed that fine-tuning at different layers of the model, i.e. early, middle and last layers, come with tackling different types of distribution shifts. In particular, \cite{lee2023surgical} showed on extensive experiments that fine tuning the last layer, corroborating the claim of \cite{kirichenko2022last}, does indeed help with spurious correlations. This is particularly important for our setting of LLMs, where reward models are given human annotated labels and hence often fall into the trap of relying on spurious features such as 'generation length'. However, we agree that future work should also consider deriving uncertainty from different layer. This is out of the scope of this paper as we mainly focus on an lightweight uncertainty estimations methods for reward modelling.  

% Having described the benefits as well as existing work on uncertainty estimation using last layer embeddings, we move on to how they can be applied to reward modelling in the RLHF pipeline. In particular, borrowing ideas from the bandit literature, we introduce an new objective during PPO which leverages uncertainty more efficiently than that of \cite{coste2023reward}.


% \subsection{Ensemble uncertainty}
% Ensemble methods are one of the most popular and most calibrated uncertainty estimation methods [add refs]. By training multiple models across different seeds, data splits or hyperparamters, ensembles are able to leverage the fact each of them learn different aspects of the data. Thus by aggregating the models and computing test statistics such as mean and standard deviation, ensembles have shown are often considered the gold-standard in terms of uncertainty estimation. This can be formalized as follows:
% \begin{align}
%     M_{\text{ENS}}(x, y) &= \frac{1}{M} \sum_{i=1}^M r^i_{\phi}(x, y)\\
%     V_{\text{ENS}}(x, y) &= \frac{1}{M} \sum_{i=1}^M \left(r^i_{\phi}(x, y) - M_{\text{ENS}}(x, y)\right)^2
% \end{align}

% However, these uncertainties do not come without cost. One prohibitive factor of ensembles is their computational requirements through training multiple models. As mentioned previously this becomes especially problematic in the setting of LLM, where models are often in the order to billions. Secondly, Ensembles are known to suffer from a diversity problem, hence making the uncertainty easily miscalibrated. To this end often times heuristics are used to induce diversity in the predictions of the models.

\paragraph{Bayesian Uncertainty.}
Bayesian uncertainty modelling, such as Bayesian Linear Regression (BLR) or Gaussian Processes (GP) \cite{williams1995gaussian}, also offers an elegant method to quantify uncertainty in closed form.

% \xy{
% This section might be placing a significant burden on readers due to a lot of notations. Could we revert to the previous notations and provide a concise description of how the uncertainty is calculated here? We can include references for those interested in further details.}

% \hnote{Not sure why we mention this as we do not have $r_i$?} \jef{these are the estimated rewards from the reward model for training data}

For simplicity of illustration, we first consider BLR in this section and subsequently describe GPs \cite{williams1995gaussian}. 
%Consider a dataset $\mathcal{D} = \{e(x_i, y_i), r_{\varphi}(x_i, y_i)\}_{i=1}^N$, where $e(x_i, y_i)$ denotes the final layer embeddings, and $r_{\varphi}(x_i, y_i)$ are the corresponding rewards from the reward model. 
In BLR, the projection weights $\phi$ are presumed to follow a Gaussian prior, expressed as $p(\phi) = \mathcal{N}(\phi | \mathbf{m}_0, \mathbf{S}_0)$, with $\mathbf{m}_0$ being the prior mean and $\mathbf{S}_0$ the prior covariance matrix.

%Given that BLR is linear in the embeddings space, 
Then the predictive posterior mean $\mu_{\text{post}}$ and variance  $\sigma^2_{\text{post}}$ of the reward for a new datapoint $(x, y)$ in BLR can be expressed in closed form as follows:
\begin{align}
p(r | x, y, \mathcal{D}) &= \mathcal{N}(r | \mu_{\text{post}}, \sigma^2_{\text{post}})\\
\mu_{\text{post}} &= e(x, y)^\top \mathbf{m}_D, \\
\sigma_{\text{post}} &= \sqrt{e(x, y)^\top \mathbf{S}_D^{-1} e(x, y) + \epsilon^2}.
\label{eq.gp_unc}
\end{align}
where $\epsilon$ is the aleatoric noise, $\mathbf{S}_D$ and $\mathbf{m}_D$ are the closed form posterior mean and variance of the projection weights $\phi$ calculated based on the reward training data $D$. 
Now that we have presented BLR, it should be noted for GPs, the mean and covariance can be derived analogously by replacing every $e(x, y)^\top e(x', y')$ computation with $k(e(x, y), e(x', y'))$, where $k$ is a kernel function. Due to space constraints, please refer to Appendix \ref{app:gp} for a comprehensive presentation of GPs and BLR.
% \xy{Please check the sentence above to verify its correctness.}
%$\Phi$ is the design matrix formed by stacking the feature vectors $e(x_i, y_i)$, $\mathbf{r}$ is the vector of outputs $r_{\varphi}(x_i, y_i)$ and $\epsilon$ being the aleatoric noise.


Note that both aforementioned uncertainty estimation methods are Mahalanobis distances \cite{mahalanobis2018generalized} in the embedding spaces, with different scaling covariances.
% \begin{align*}
% \mathbf{S}_N^{-1} &= \mathbf{S}_0^{-1} + \Phi^T \Phi / \sigma^2, \\
% \mathbf{m}_N &= \mathbf{S}_N (\mathbf{S}_0^{-1} \mathbf{m}_0 + \Phi^T \mathbf{r} / \sigma^2),
% \end{align*}

% Note, however the caveat of BLR which is that of the inverse in $S_N$ which is of the order of $\mathcal{O}(d^3)$ where $d$ is the dimension of the embeddings. 
% \xy{How $\mathbf{m}_N$ and $\mathbf{S}_N$  are calculated? Which portion is considered the uncertainty? }

% \xy{Might I suggest that discussing 'why the last layer and not any other layer' could be more fitting under the sections for limitations or future work? Its placement here could possibly divert from the main focus. } \jef{will intergrate the below tmr. not sure if we want that much detail}







% The predictive distribution for a new $(x^*, y^*)$ is given by:
% \begin{align*}
% p(r^* | x^*, , y^* \mathcal{D}) &= \mathcal{N}(r^* | \mu_{\text{post}}, \sigma^2_{\text{post}})\\
% \mu_{\text{post}} &= \phi(x^*, y^*)^T \mathbf{m}_N, \\
% \sigma^2_{\text{post}} &= \phi(x^*, y^*)^T \mathbf{S}_N \phi(x^*, y^*) + \sigma^2.
% \end{align*}
% Here, $\mu_{\text{post}}$ and $\sigma^2_{\text{post}}$ represent the posterior mean and variance of the predictive distribution for the reward.

\subsection{Empirical Effectiveness of Lightweight Uncertainty Estimation}
\label{subsec-expun}
We empirically investigate the effectiveness of the two lightweight uncertainty estimation methods introduced in Section \ref{subsec:un-cal}. 
Since our objective is to harness uncertainty in reward modelling to mitigate the overoptimization issue in RLHF, we specifically examine whether the two approaches can identify discrepancies between estimated proxy rewards and gold rewards during the RL stage. 
We adopt a synthetic setup widely used in the literature \cite{gao2023scaling,coste2023reward, eisenstein2023helping}, where we train a significantly larger ``\textit{gold-standard}" reward model that simulates human preferences and provides labels for training a proxy reward model.


We run a standard RLHF pipeline on the Anthropic HH \cite{bai2022training} and TL;DR dataset\cite{stiennon2020learning}, with reward and policy models established from LLama-7B \cite{touvron2023llama}.
The preference dataset is labelled by the gold reward model. In particular, for the Anthropic HH dataset, the gold reward model is trained from Vicuna-13B \cite{platzer_et_al:LIPIcs.ECRTS.2021.1}, and for the TL;DR dataset, the gold reward model is trained from LLama-13B \cite{touvron2023llama}. Additional details, such as gold/proxy reward model training, PPO implementation, etc., can be found in Appendix \ref{appedix:exp-syn}.
% experimental procedurefor gold reward training 

% To simulate the fact that in a real setup, human preferences are too
% complex to be captured by a neural network with a finite
% capacity, we employ larger LLMs to get the gold reward models following previous work[ref]. 

During the PPO training stage, we log the generated samples every 10 steps. Subsequently, we compute their gold reward, proxy reward, as well as reward uncertainties associated with the proxy reward.
We compare the following uncertainty methods: 
\squishlist
 \item \textbf{CI}: 
 The uncertainty quantified 
 %Confidence Interval (CI) 
 through Eq.(\ref{inequ:bandit-un}); 
 \item \textbf{GP}: Gaussian Process uncertainty through Eq.(\ref{eq.gp_unc}); 
\item \textbf{ENS-7B}:  Ensemble of three LLama7B reward models; 
\item \textbf{ENS-3B}: Ensemble of three 3B reward models based on OpenLLaMA3B\_v2 \cite{openlm2023openllama}. Since there are no officially released 3B models for LLaMA, we adopt OpenLLaMA \cite{openlm2023openllama} which is an open-source smaller reproduction of Meta AI’s LLaMA, showcasing comparable performance.
\squishend

The results are presented in Figure \ref{fig:un}. In Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff}, we depict the correlation between derived uncertainty\footnote{Uncertainties calculated by different methods have different scales, so we normalized them to (0,1) for ease of comparison.} and the difference between gold reward and proxy reward (i.e., $|r^*(x,y) - r_{\varphi}(x,y)|$). Ideally, an effective uncertainty measure should increase as the difference between gold and proxy reward increases.
In Figure \ref{fig:hh-un-step} and Figure \ref{fig:tldr-un-step}, we illustrate the progression of proxy rewards (blue dashed line), gold rewards (blue solid line), and uncertainties calculated by two lightweight uncertainty estimation methods, along with ENS-3B, 
throughout the PPO optimization steps. The reward values are indexed on the left y-axis, while the uncertainty is indexed on the right y-axis. These figures provide insight into whether the calculated uncertainties can effectively recognize the over-optimization issue.

Our key insights are summarized as follows:

\begin{figure*}[t]
  \centering
  % \vspace{-5mm}
  \subfloat[Anthropic HH (Step)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/ANT_UN_step.png}
             \label{fig:hh-un-step}}
    \subfloat[Anthropic HH (Reward Diff)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/ANT_UN_reward_diff.png}
             \label{fig:hh-un-rewarddiff}}
   \subfloat[TL;DR (Step)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/TLDR_UN_step.png}
             \label{fig:tldr-un-step}}
  \subfloat[TL;DR (Reward Diff)]
           { \includegraphics[width=.24\linewidth, height=.18\linewidth]{figures/TLDR_UN_reward_diff.png}
             \label{fig:tldr-un-rewarddiff}}
% \vspace{-1mm}
    \caption{Comparison among lightweight uncertainty estimations. In Figure \ref{fig:hh-un-step} and \ref{fig:tldr-un-step}, the blue lines with shaded areas depict the reward dynamics concerning optimization steps in PPO, where the solid and dashed lines represent gold and proxy rewards, respectively. The lines with dots denote the results from different uncertainty estimation methods. The reward values are indexed on the left y-axis, while the uncertainty is indexed on the right y-axis. In Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff}, we plot the correlation between uncertainty and the difference between gold reward and proxy reward.}
    \label{fig:un}
% \vspace{-4mm}
\end{figure*}


\noindent\textit{$\bullet$ The lightweight uncertainty estimation methods are effective in signalling over-optimizaton.} 
We observe from Figure \ref{fig:hh-un-rewarddiff} and \ref{fig:tldr-un-rewarddiff} that, as the difference between gold reward and proxy reward increases, the uncertainty calculated by CI and GP also rises. This demonstrates CI and GP indeed carry information on when the proxy reward is drifting away from the ground-truth reward. 
Furthermore, in Figure \ref{fig:hh-un-step} and \ref{fig:tldr-un-step}, it is evident that when there is a divergence between golden and proxy rewards, indicating over-optimization, the uncertainty calculated by CI and GP generally increases with the optimization steps. This suggests the potential to leverage them to address the over-optimization issue. CI appears to outperform GP since it consistently increases with the divergence of gold and proxy rewards, while GP tends to stabilize after roughly $500$ steps, as shown in Figure \ref{fig:tldr-un-step}.



\noindent\textit{$\bullet$ The lightweight uncertainty estimation surpasses reward ensembles with comparable parameter sizes. }  Compared to the two lightweight uncertainty estimation methods, ENS-3B appears to be less correlated with the divergence between gold and proxy rewards, particularly on the TL;DR dataset \cite{stiennon2020learning}. Contrary to our lightweight uncertainty estimation methods, the uncertainty calculated by ENS-3B does not exhibit a monotonically increasing trend with the reward difference between gold and proxy rewards. This is likely due to the fact the smaller reward models, in this case, 3B models, are not able to capture the preference well, thus leading to worse predictions.


